Lifting the Information Ratio: An Information-Theoretic Analysis of Thompson Sampling for Contextual Bandits

We study the Bayesian regret of the renowned Thompson Sampling algorithm in contextual bandits with binary losses and adversarially-selected contexts. We adapt the information-theoretic perspective of \cite{RvR16} to the contextual setting by considering a lifted version of the information ratio defined in terms of the unknown model parameter instead of the optimal action or optimal policy as done in previous works on the same setting. This allows us to bound the regret in terms of the entropy of the prior distribution through a remarkably simple proof, and with no structural assumptions on the likelihood or the prior. The extension to priors with infinite entropy only requires a Lipschitz assumption on the log-likelihood. An interesting special case is that of logistic bandits with $d$-dimensional parameters, $K$ actions, and Lipschitz logits, for which we provide a $\widetilde{O}(\sqrt{dKT})$ regret upper-bound that does not depend on the smallest slope of the sigmoid link function.

==> 3-results-edit.tex <==
\section{Main results}
In this section, we state our main results concerning the Bayesian regret of Thompson sampling for contextual bandits. 
We begin by stating two general regret bounds in terms of the lifted information ratio defined in Equation~\eqref{eq:RIR}. 
The reader that is not interested in the full generality of our theory may skip to Section~\ref{sec:concrete} for concrete regret bounds in practical settings.

Our first abstract bound applies to priors with finite entropy, the simplest example being finite parameter spaces. 
\begin{thm}\label{th:main_discrete}
	Assume $Q_0$ is supported on the countable set $\Theta_0 \subseteq \Theta$ and that the lifted information 
	ratio for all rounds $t$ satisfies $\rho_t \le \rho$ for some $\rho > 0$. Then, the Bayesian regret of \TS after $T$ 
	rounds can be bounded as
	\begin{equation*}
	R_T \le \sqrt{\rho TH(\theta^\star)},
	\end{equation*}
	where $H(\theta^\star)=-\EE{\theta^\star\sim Q_0}$  
	is the Shannon entropy of the prior 
	distribution\todoG{Maybe we can define this earlier since it is mentioned several times before?}. In particular if $\Theta_0$ is a finite set with $|\Theta_0|=N$, the regret of \TS satisfies
	\begin{equation*}
	R_T \le \sqrt{\rho T\log N}. %= \wt{O}(\sqrt{KT}).
	\end{equation*}
\end{thm}

Unfortunately, the Shannon entropy can be unbounded for distributions with infinite support, which is in fact the 
typical situation that one encouters in practice. 
To address this concern, we develop a more general result, that holds for a broader family of distributions. 
In the following, $(\Theta, \varrho)$ is a metric space with metric $\varrho:\Theta^2\to\Reals$.
We make the following regularity assumption on the log-likelihood function $P_{\theta,x,a}$:
\begin{assumption}\label{ass:log_lipschitz}
	There exists a constant $C>0$ such that for any  $\theta, \theta' \in \Theta$, 
	$\abs{\log P_{\theta,x,a}(r) - \log P_{\theta',x,a}(r)} \le C \varrho(\theta, \theta')$ holds for all 
	$x\in\X$, $a\in\mathcal{A}$, and $r\in\{0,1\}$. 
\end{assumption}
Under this assumption, we can state a variant of Theorem~\ref{th:main_discrete} that applies to metric parameter 
spaces:
\begin{thm}\label{th:main_continuous}
	Assume $(\Theta, \varrho)$ is a metric space, and $Q_0$ is supported on $\Theta_0\subseteq\Theta$ with 
	$\epsilon$-covering number $\mathcal{N}_{\epsilon}(\Theta_0,\varrho)$. Let Assumption~\ref{ass:log_lipschitz} hold, and 
	assume the lifted information ratio for all rounds $t$ satisfies $\rho_t \le \rho$ for some 
	$\rho > 0$. Then, the Bayesian regret of \TS after $T$ rounds can be bounded as
	\begin{equation*}
	R_T \le \sqrt{\rho T\left(\log\left(\mathcal{N}_{1/(CT)}(\Theta_0,\varrho)\right)+1\right)}.
	\end{equation*}
\end{thm}

To get a better understanding of Assumption~\ref{ass:log_lipschitz}, it is useful to notice that it is satisfied in 
basic settings like linear and logistic bandits, as we will show in Section~\ref{sec:concrete}.
However, at this point, some readers may worry that the lifted information ratio may be impossible to bound due to the lifting to the space of parameters $\Theta$. Our next step will be to bound the lifted information ratio for three problem settings of practical interest.

\subsection{Bounds on the lifted information ratio}
The first setting we consider is that of contextual bandits with finite actions and binary losses. 

\begin{lemma}\label{lem:ir_finite}
Suppose that the losses take values in $\ev{0,1}$ and the actions space is finite with $|\mathcal{A}|=K$. Then, the lifted information ratio of Thompson sampling satisfies 
$\rho_t \le 2K$.
\end{lemma}


Then, we consider the case of linear losses in Euclidean parameter spaces, which allows continuous actions.\todo{M: is this last part about infinite actions correct?}
\begin{lemma}\label{lem:ir_linear}
Suppose that $\Theta\subseteq\real^d$ and the expected losses are linear functions of the form $\ell(\theta,x,a) = 
\iprod{\theta}{\varphi(x,a)}$, where $\varphi:\mathcal{X}\times[K]\ra \real^d$ is a feature map. Then, the lifted 
information ratio satisfies $\rho_t \le d$.
\end{lemma}
\gcomment{Julia can you check that this is true in this form or do we need some more assumptions?}

Finally, for the case of many (but still finite) actions, we consider an alternative condition on the loss distribution.
\redd{\begin{lemma}\label{lem:ir_subgauss}\todoG{Lots of wishful thinking here!!! I have no idea if this is true but it 
would be lovely.}
Suppose that for each $t$, the conditional distribution $\ell(\theta^\star,x,a)|\F_{t-1}$ is $\alpha_t$-subgaussian and 
has standard deviation $\sigma_t$. Then, the lifted information ratio satisfies $\rho_t \le 
\pa{\frac{\alpha_t}{\sigma_t}}^2 \log K$.
\end{lemma}}
This last assumption is satisfied in the standard Bayesian linear bandit setting where the prior and posterior distributions 
are Gaussian, so that the ratio $\alpha_t / \sigma_t$ equals 1.
We will now turn to concrete examples.

\subsection{Concrete regret bounds}\label{sec:concrete}
We start from a basic setting: finite actions, binary losses, and finitely-supported prior. The following regret bound follows directly from Theorem~\ref{th:main_discrete} and Lemma~\ref{lem:ir_finite}.
\begin{cor}
	Consider a contextual bandit with $K$ actions and binary losses, and suppose $\Theta_0$, the support of $Q_0$, is finite with $|\Theta_0|=N $. Then, the Bayesian regret of \TS satisfies:
	\begin{equation*}
	R_T \le \sqrt{KT\log N}.
	\end{equation*}
\end{cor}

As a more practical setting, we consider linear bandits with bounded parameters and features. Here $\Theta\subseteq\Reals^d$ and losses are generated by a Gaussian distribution $L_t \sim \mathcal{N}(\langle \theta^{\star},\varphi(X_t,A_t)\rangle, \sigma^2)$, where $\varphi:\X\times\mathcal{A}\to\Reals^d$ is a feature map. We will assume $\sigma=1$ for simplicity. 
We essentially recover the classic regret bounds for this setting---see, e.g., \cite{APS11}\todo{M: complete the references}---of order $d\sqrt{T\log\pa{RST}}$ for infinite actions and $\sqrt{dT\log\pa{KRST}}$ for many (finite) actions.
\begin{cor}
	Consider the class of $d$-dimensional linear bandits with bounded features and parameters. Let $R = \sup_{x,a} \norm{\varphi(x,a)}$\todo{let's use a better $R$ for the regret then, like $\mathcal{R}$} and $S = 
	\sup_{\theta \in\Theta} \norm{\theta}$. Then, the Bayesian regret of \TS satisfies
	\begin{equation}
		R_T \le d\sqrt{T(\log(2RST+1)+1)}.
	\end{equation}
	{\color{red}
		Moreover, if $|\mathcal{A}|=K$,
		\begin{equation}
		R_T \le \sqrt{T\log(K)(\log(2RST+1)+1)}.
		\end{equation}
	}
\end{cor}
We obtained this result as a special case of Theorem~\ref{th:main_continuous} under a variant of Assumption~\ref{ass:log_lipschitz} that allows the Lipschitz constant to depend on the loss. We used an $\wt{O}(d)$ log-covering number, by standard covering of the Euclidean ball. As for the lifted information ratio, both Lemma~\ref{lem:ir_linear} \redd{and Lemma~\ref{lem:ir_subgauss}} apply here. 
We defer the complete proof to \redd{the appendix}. 

\todo{M: check the Lipschitz constant for the Gaussian case!}

An even more interesting setting is that of logistic bandits.
% This  is referred as logistic bandits in the sequential learning literature~\citep{FCGS10,LLZ17,FACF20,AFC21, FAJC22}.
% 
% \paragraph{Logistic bandits.}
In this model, the losses are generated by a Bernoulli distribution as $L_t(\theta, x, a) \sim 
Ber(\sigma(f_{\theta}(x,a)) )$, where $\sigma(f_{\theta}(x,a)) = \frac{1}{1+ \exp(-f_{\theta}(x,a) )}$ and 
$f_{\theta}(x,a)$, called the logit function, is $C$-Lipschitz in $\theta$. 
Notice that our definition generalizes the commonly used notion of logistic bandits, popularized by~\citet{FCGS10}\todo{M:check if this is historically correct}, that consider linear logit 
functions of the form $f_{\theta}(x,a)=\langle\theta,\varphi(x,a)\rangle$, where 
$\varphi:\X\times\mathcal{A}\to\Reals^d$ is 
some feature map. 
Our result for logistic bandits is also based on Theorem~\ref{th:main_continuous}.
\begin{cor}\label{th:main_logistic}
	Assume $\Theta\subset\Reals^d$ and $\norm{\theta}\le S$ for all $\theta\in\Theta_0$. Consider a class of logistic 
bandits with $C$-Lipschitz logit function $f_{\theta}(x,a)$. Also, assume that the lifted information ratio for all 
rounds $t$ satisfies $\rho_t \le \rho$ for some 
	$\rho > 0$.\todo{M: not introducing the finite-action asm here in the hope we can prove the other bound for the linear case} Then, the Bayesian regret of \TS after $T$ rounds can be bounded as:
	\begin{equation*}
	R_T \le \sqrt{\rho T\left(d\log(2SCT + 1)+1\right)}.
	\end{equation*}
\end{cor}
\begin{proof}
	Here $\Theta$ equipped with the Euclidean norm $\norm{\cdot}$ is our metric space, and $\Theta_0$ is contained in the Euclidean ball of radius $S$. %	
	Using a standard result on the covering number of the Euclidean ball~\citep{xx} we have $\mathcal{N}_\varepsilon(\Theta_0,\norm{\cdot}) \le (\frac{2S}{\varepsilon}+1)^d$. 
	Regarding Assumption~\ref{ass:log_lipschitz}, notice that $\log(\sigma(f_{\theta}(x,a))) = 
	f_{\theta}(x,a) - \log(1+\exp(f_{\theta}(x,a)))$. Since $\log(\sigma(z))$ and $\log(1-\sigma(z))$ are $1$-Lipschitz and $f_{\theta}(x,a)$ is $C$-Lipschitz, 
	$\log P_{\theta,x,a}(1)=\log(\sigma(f_{\theta}(x,a)))$ and $\log ˘P_{\theta,x,a}(0)=\log(1-\sigma(f_{\theta}(x,a)))$ are also $C$-Lipschitz, implying that 
	Assumption~\ref{ass:log_lipschitz} holds with the same constant $C$. 
	The claim then follows from Theorem~\ref{th:main_continuous}.
\end{proof}\todoG{Move this to the analysis section or the appendix to preserve the flow.}
% Instead, we allow nonlinear logit functions, provided they are Lipschitz.
% Even more generally, Assumption~\ref{ass:log_lipschitz} holds for any functions with a range within $(0,1)$: 
% \paragraph{Bounded functions.} For any  $L$-Lipschitz function $f_{\theta}(x,a)$ with a range $[a,b]$ \todo{J: still 
% that odd thing that $p_\theta(L_t)$ cannot be small} for some $0<a\le b<1$, $\log(f_{\theta}(x,a))$ and $\log(1 - 
% f_{\theta}(x,a))$ are $C$-Lipschitz with $C=\max \{\frac{1}{a}, \frac{1}{1-b}\}$.
We can further specialize it to logistic bandits with linear logits {\color{red} and finite actions}:
\begin{cor}\label{th:main_linear_logit}
	Assume $\Theta\subset\Reals^d$, $\norm{\theta}\le S$ for all $\theta\in\Theta$, and $\mathcal{A}=[K]$. Consider a class of logistic bandits with linear logit function $f_{\theta}(x,a)=\langle\varphi(x,a),\theta\rangle$, with $\norm{\phi(x,a)}\le B$ for all $x\in\X$ and $a\in[K]$. Then, the Bayesian regret of \TS after $T$ rounds can be bounded as:
	\begin{equation*}
	R_T \le \sqrt{2KT\left(d\log(2SBT+1)+1\right)} = \wt{O}\big(\sqrt{dKT}\big).
	\end{equation*}
\end{cor}
\begin{proof}
	The function $f_{\theta,x,a} : \theta \to \langle\varphi(x,a),\theta\rangle$ is linear in $\theta$ and since $\varphi(x,a)$ is bounded in norm by B, it is also $B$-Lipschitz.
	This proves that Assumption~\ref{ass:log_lipschitz} is satisfied with the constant $B$. We can then apply Corollary \ref{th:main_logistic} with $C=B$ and $\rho=K$ (Lemma~\ref{lem:ir_finite}).
\end{proof}
\todo[inline]{Comparison with existing results on linear logits: easier if we remove the $K$ factor!}
\gcomment{It would surely make our result look good, but not it's not necessarily fair. Indeed it seems that one has to 
pay a big price to go to infinite action spaces and this should be discussed nicely.}
\gcomment{TODO: prove another bound on the information ratio for this setting---perhaps scaling with the smallest 
slope.}


%TODO: mover to proof section:
%Moreover, in the Bayesian setting, the posterior-sample parameter $\theta_t$ has the same distribution as 
%$\theta^\star$ conditional on $\F_{t-1}$. This means $(\theta_t, A_t)$ has the same distribution as $(\theta^\star, 
%A^\star_t)$ conditional on $\F_{t-1}$ and $X_t$. Notice how $\theta_t$ and $A_t$ are dependent random variables, and so 
%are $\theta^\star$ and $A^\star_t$, but $(\theta_t, A_t)$ is conditionally independent from $(\theta^\star, A^\star_t)$. 
%We will use these properties of \TS in the proofs of Section~\ref{sec:theory}.



==> 3-results_g.tex <==
\section{Main results}
In this section, we state our main results concerning the Bayesian regret of Thompson sampling for contextual bandits. 
We will assume that the losses are binary and the action space is finite, unless otherwise stated. However, several 
of our results can be generalized beyond this setting, as we will illustrate this in Section~\ref{sec:gaussian} where 
we provide some additional results for the classic setting of Gaussian linear contextual bandits.

We begin by stating two general regret bounds in terms of the \IR defined in Equation~\eqref{eq:RIR}. 
The reader that is not interested in the full generality of our theory may skip to Section~\ref{sec:concrete} for concrete regret bounds.
Our first abstract bound applies to priors with finite entropy, the simplest example being finite parameter spaces. 
\begin{thm}\label{th:main_discrete}
	Assume $Q_0$ is supported on the countable set $\Theta_0 \subseteq \Theta$ and that the \IR for all rounds $t$ satisfies $\rho_t \le \rho$ for some $\rho > 0$. Then, the Bayesian regret of \TS after $T$ 
	rounds can be bounded as
	\begin{equation*}
	R_T \le \sqrt{\rho TH(\theta^\star)},
	\end{equation*}
	where $H(\theta^\star)=-\EE{\theta^\star\sim Q_0}$  
	is the Shannon entropy of the prior 
	distribution\todoG{Maybe we can define this earlier since it is mentioned several times before?}. In particular if $\Theta_0$ is a finite set with $|\Theta_0|=N$, the regret of \TS satisfies
	\begin{equation*}
	R_T \le \sqrt{\rho T\log N}. %= \wt{O}(\sqrt{KT}).
	\end{equation*}
\end{thm}
Unfortunately, the Shannon entropy can be unbounded for distributions with infinite support, which is in fact the 
typical situation that one encouters in practice. 
To address this concern, we develop a more general result, that holds for a broader family of distributions. 
In the following, $(\Theta, \varrho)$ is a metric space with metric $\varrho:\Theta^2\to\Reals$.
We make the following regularity assumption on the likelihood function $P_{\theta,x,a}$:
\begin{assumption}\label{ass:log_lipschitz}
	There exists a constant $C>0$ such that for any  $\theta, \theta' \in \Theta$, 
	$\abs{\log P_{\theta,x,a}(r) - \log P_{\theta',x,a}(r)} \le C \varrho(\theta, \theta')$ holds for all 
	$x\in\X$, $a\in\mathcal{A}$, and \redd{$r\in\{0,1\} $}.\todo{J: need to define the set of outcomes and replace 
$\{0,1\} $ here by that set} \todoG{I suggest we stay with $\ev{0,1}$ to keep things simple and consistent here.}
\end{assumption}
Under this assumption, we can state a variant of Theorem~\ref{th:main_discrete} that applies to metric parameter 
spaces:
\begin{thm}\label{th:main_continuous}
	Assume $(\Theta, \varrho)$ is a metric space, and $Q_0$ is supported on $\Theta_0\subseteq\Theta$ with 
	$\epsilon$-covering number $\mathcal{N}_{\epsilon}(\Theta_0,\varrho)$. Let Assumption~\ref{ass:log_lipschitz} hold, and 
	assume the \IR for all rounds $t$ satisfies $\rho_t \le \rho$ for some 
	$\rho > 0$. Then, the Bayesian regret of \TS after $T$ rounds can be bounded as
	\begin{equation*}
	R_T \le \sqrt{\rho 
T\textstyle{\min_{\varepsilon}}\left(\log\left(\mathcal{N}_{\varepsilon}(\Theta_0,\varrho)\right)+\varepsilon 
CT\right)}.
	\end{equation*}
\end{thm}
To get a better understanding of Assumption~\ref{ass:log_lipschitz}, it is useful to notice that it is satisfied in 
basic settings, like logistic bandits with Lipschitz logits. See Section~\ref{sec:concrete} for details.

\subsection{Bounding the \IR}
At this point, some readers may worry that the \IR may be impossible to bound due to the lifting 
to the space of parameters $\Theta$. To address this concern, we now turn to showing bounds on the \IR.
We first consider the unstructured case, that holds for arbitrary parameter spaces $\Theta$, likelihoods, and priors.
\begin{lemma}\label{lem:ir_finite}
Suppose that the losses are binary and $|\mathcal{A}|=K$. Then, the 
\IR of Thompson sampling satisfies $\rho_t \le 2K$ for all $t\ge 1$.
\end{lemma}
The proof of this lemma (provided in Section~\ref{sec:IRbound}) relies on a decoupling argument between the choice of 
the action and of the parameters at round $t$, inspired by \citet{Zha21}. Taking his argument one step further, we 
center our analysis around an application of convex conjugacy, which we believe may be applicable in a broader variety 
of settings. We wish to highlight that this proof technique is very different from the information-theoretic 
methodology pioneered by \citet{RvR16}.

Next, we consider the case of linear expected losses in Euclidean parameter spaces, which, in principle, allows for an 
unbounded number of actions.
\begin{lemma}\label{lem:ir_linear}
Suppose that $\Theta\subseteq\real^d$, the losses are binary, and the expected losses are linear functions of the form 
$\ell(\theta,x,a) = \iprod{\theta}{\varphi(x,a)}$, where $\varphi:\mathcal{X}\times\mathcal{A}\ra \real^d$ is a feature 
map. Then, the \IR satisfies $\rho_t \le d$.
\end{lemma}\todo{M: make sure the proof of Lemma 2 is stated for the bounded-loss case, that is with (Pinsker) inequality and not equality in the first step}
The proof of this result follows the arguments of Proposition~5 of \citet{RvR16}, with some small but important 
changes to account for the presence of contexts. 

Notably, both of these results match the classic bounds of~\citet{RvR16} on the standard definition of the 
information ratio for these settings (cf.~their Propositions~5 and~3) up to constant factors, implying that lifting to 
the space of parameters does not substantially impact the regret-information tradeoff in this setting. 
\todo[inline]{M: should we anticipate the fact that for gaussian losses with linear expected losses 
$\rho\le\min\{d,\log K\}$ ? \gcomment{I tried to write a sentence about it but it felt clumsy so maybe we better not 
mention this now.}}

%TODO: the LIR bound from lemma 3 will only be stated for the Gaussian case in its dedicated section
%Finally, for the case of many (but still finite) actions, we consider an alternative condition on the loss distribution.
%\redd{\begin{lemma}\label{lem:ir_subgauss}
%Suppose that for each $t$, the conditional distribution $\ell(\theta^\star,x,a)|\F_{t-1}$ is $\alpha_t$-subgaussian and 
%has standard deviation $\sigma_t$. Then, the \IR satisfies $\rho_t \le 
%\pa{\frac{\alpha_t}{\sigma_t}}^2 \log K$.
%\end{lemma}}
%This last assumption is satisfied in the standard Bayesian linear bandit setting where the prior and posterior 
%distributions are Gaussian, so that the ratio $\alpha_t / \sigma_t$ equals 1.

\subsection{Concrete regret bounds for Bernoulli bandits}\label{sec:concrete}
We now instantiate our bounds in two well-studied settings for Bernoulli bandits. 
We start from the fully unstructured case, assuming finite actions and finitely supported prior. The following regret bound follows directly from 
Theorem~\ref{th:main_discrete} and Lemma~\ref{lem:ir_finite}.
\begin{thm}
	Consider a contextual bandit with $K$ actions and binary losses, and suppose $\Theta_0$, the support of $Q_0$, is finite with $|\Theta_0|=N $. Then, the Bayesian regret of \TS satisfies:
	\begin{equation*}
	R_T \le \sqrt{KT\log N}.
	\end{equation*}
\end{thm}
This result is comparable to the best known results due to \citet{FK21} (for the FastCB algorithm) and \citet{Zha21} (for a novel Bayesian algorithm), and matches the 
minimax rate for unstructured contextual bandits with a policy class of size $N$~\citep{ADKLS12}. However, we are not aware of a comparable 
result for the Thompson sampling algorithm in the literature, be it Bayesian or frequentist regret.
\gcomment{Cite Exp4 and some John Langford papers?}

Moving to Bernoulli bandits with structure, we consider a well-studied setting known as logistic bandits.
In this model, the losses are generated by a Bernoulli distribution as $L_t(\theta, x, a) \sim 
Ber(\sigma(f_{\theta}(x,a)) )$, where $\sigma(z) = 1/(1+ e^{-z})$ is the sigmoid function. We just assume that $f_{\theta}(x,a)$, called the logit function, is $C$-Lipschitz in $\theta$. 
Notice that our definition generalizes the commonly used notion of logistic bandits~\citep{FCGS10,LLZ17,FACF20,AFC21, FAJC22}, that consider linear logit 
functions of the form $f_{\theta}(x,a)=\langle\theta,\varphi(x,a)\rangle$, where 
$\varphi:\X\times\mathcal{A}\to\Reals^d$ is 
some feature map. 
Our result for logistic bandits is also based on Theorem~\ref{th:main_continuous}.

\begin{thm}\label{th:main_logistic}
	Assume $\Theta\subset\Reals^d$ and $\norm{\theta}\le S$ for all $\theta\in\Theta_0$. Consider a class of logistic 
bandits with $K$ actions and $C$-Lipschitz logit function $f_{\theta}(x,a)$. Then, the Bayesian regret of \TS after $T$ rounds can be bounded as:
	\begin{equation*}
	R_T \le \sqrt{K T\left(d\log(2SCT + 1)+1\right)}.
	\end{equation*}
\end{thm}
\redd{To our knowledge, this is the first regret bound for logistic bandits with nonlinear logits.}\todo{M: is this true?}

%TODO: move proof to the appendix
%\begin{proof}
%	Here $\Theta$ equipped with the Euclidean norm $\norm{\cdot}$ is our metric space, and $\Theta_0$ is contained in the Euclidean ball of radius $S$. %	
%	Using a standard result on the covering number of the Euclidean ball~\citep{xx} we have $\mathcal{N}_\varepsilon(\Theta_0,\norm{\cdot}) \le (\frac{2S}{\varepsilon}+1)^d$. 
%	Regarding Assumption~\ref{ass:log_lipschitz}, notice that $\log(\sigma(f_{\theta}(x,a))) = 
%	f_{\theta}(x,a) - \log(1+\exp(f_{\theta}(x,a)))$. Since $\log(\sigma(z))$ and $\log(1-\sigma(z))$ are $1$-Lipschitz and $f_{\theta}(x,a)$ is $C$-Lipschitz, 
%	$\log P_{\theta,x,a}(1)=\log(\sigma(f_{\theta}(x,a)))$ and $\log ˘P_{\theta,x,a}(0)=\log(1-\sigma(f_{\theta}(x,a)))$ are also $C$-Lipschitz, implying that 
%	Assumption~\ref{ass:log_lipschitz} holds with the same constant $C$. 
%	The claim then follows from Theorem~\ref{th:main_continuous}.
%\end{proof}

% Instead, we allow nonlinear logit functions, provided they are Lipschitz.
% Even more generally, Assumption~\ref{ass:log_lipschitz} holds for any functions with a range within $(0,1)$: 
% \paragraph{Bounded functions.} For any  $L$-Lipschitz function $f_{\theta}(x,a)$ with a range $[a,b]$ \todo{J: still 
% that odd thing that $p_\theta(L_t)$ cannot be small} for some $0<a\le b<1$, $\log(f_{\theta}(x,a))$ and $\log(1 - 
% f_{\theta}(x,a))$ are $C$-Lipschitz with $C=\max \{\frac{1}{a}, \frac{1}{1-b}\}$.
We can further specialize our result to logistic bandits with linear logits, the setting that is most commonly studied in the literature:
\begin{cor}\label{th:main_linear_logit}
	Assume $\Theta\subset\Reals^d$, $\norm{\theta}\le S$ for all $\theta\in\Theta$. Consider a class of logistic bandits with $K$ actions and linear logit function $f_{\theta}(x,a)=\langle\varphi(x,a),\theta\rangle$, with $\norm{\phi(x,a)}\le B$ for all $x\in\X$ and $a\in[K]$. Then, the Bayesian regret of \TS after $T$ rounds can be bounded as:
	\begin{equation*}
	R_T \le \sqrt{2KT\left(d\log(2SBT+1)+1\right)} = \wt{O}\big(\sqrt{dKT}\big).
	\end{equation*}
\end{cor}

%TODO: move proof to appendix
%\begin{proof}
%	The function $f_{\theta,x,a} : \theta \to \langle\varphi(x,a),\theta\rangle$ is linear in $\theta$ and since $\varphi(x,a)$ is bounded in norm by B, it is also $B$-Lipschitz.
%	This proves that Assumption~\ref{ass:log_lipschitz} is satisfied with the constant $B$. We can then apply Corollary \ref{th:main_logistic} with $C=B$ and $\rho=K$ (Lemma~\ref{lem:ir_finite}).
%\end{proof}

This result matches the one by~\citet{DMvR19} on Thompson sampling if we naively upper bound the fragility dimension with the number of actions, which is the best we can do without further assumptions on the structure of the problem.\todo{M: this is the best comparison I could come up with so far, I still found all the assumptions from that paper bizarre.}
An alternative bound for the many-actions setting that scales almost logarithmically with $K$ remains an open problem. Its difficulty is testified by the negative examples provided by~\citet{DMvR19}, and by the long-lived conjecture from~\citep{DvR18}, that, to our knowledge, has not yet been verified in theory. However, this kind of bound is known to hold for \emph{linear} bandits~\citep[e.g.,][]{BCK12}, and our framework allows to recover it when the noise is Gaussian, as we will now show.

\subsection{Beyond binary losses: linear bandits with Gaussian noise}
We next consider the classic setting of linear bandits, where the loss is a linear function of a $d$-dimensional feature map of context and action.
We essentially recover the classic regret bounds for this setting---see, e.g., \cite{APS11,BCK12}, that obtain a regret bound of order $\sqrt{dT\log K}$.

\begin{cor}
 Consider the classic setting of linear bandits, such that the loss of playing action $a$ at time $t$ satisfies 
	$\ell(\theta^*, x, a) \sim \mathcal{N}(\langle 
	\theta^{\star},\varphi(x,a)\rangle, \sigma^2)$, where $\theta^*$ is drawn from a Gaussian prior
	$Q_1 =  \mathcal{N}(0, \lambda I )$ with some $\lambda >0$, $\sigma >0$  and $\varphi:\X\times[K]\to\Reals^d$ is a feature map 	such that $ 
	\norm{\varphi(x,a)} \le B$ for all $x\in \X, a \in [K]$.  Then, the Bayesian regret of TS satisfies
	\[ \EE{R_T} \le \sqrt{ 2d T  \min\{2(1+\log K),d\}  \log\pa{1+ \frac{ T\lambda B^2 }{d \sigma^2}}}   .\]
\end{cor}

While for the cases when $d \ll \log K$ the dependence on $K$ is not present in the regret bound, our analysis is restricted to the setting with the finite number of actions. Still, using a standard discretization argument, 
 it is possible
expand the analysis for an infinite action space. 


%TODO: mover to proof section:
%Moreover, in the Bayesian setting, the posterior-sample parameter $\theta_t$ has the same distribution as 
%$\theta^\star$ conditional on $\F_{t-1}$. This means $(\theta_t, A_t)$ has the same distribution as $(\theta^\star, 
%A^\star_t)$ conditional on $\F_{t-1}$ and $X_t$. Notice how $\theta_t$ and $A_t$ are dependent random variables, and so 
%are $\theta^\star$ and $A^\star_t$, but $(\theta_t, A_t)$ is conditionally independent from $(\theta^\star, A^\star_t)$. 
%We will use these properties of \TS in the proofs of Section~\ref{sec:theory}.



==> 4-analysis_continious.tex <==
\section{Analysis}\label{sec:theory}

We use $g$ to denote the binary relative entropy function:
\begin{equation}\label{eq:bin_relent}
g(p\|q) = p\log\frac{p}{q} + (1-p)\log\frac{1-p}{1-q},
\end{equation}
where $p,q\in[0,1]$ and we use the convention $0\cdot\log 0 = 0$. By $g^*$ we always mean the Fenchel dual of $g$ w.r.t. its first argument, that is:\todo{should we include a proof of this?}
\begin{equation}
g^*(u\|q) = \log(1+q(e^u - 1)),
\end{equation}
where $u\in\Reals$ and $q\in[0,1]$.
The following upper bound on the dual of the relative entropy will be useful:
\begin{proposition}\label{prop:dual_bound}
	For any $u\le 0$\todo{We only apply it to negative dual variable, which gives us the $1/2$ factor in the quadratic term} and $q\in[0,1]$:
	\begin{equation*}
	g^*(u\|q) \le q\left(u + \frac{u^2}{2}\right).
	\end{equation*}
\end{proposition}
\begin{proof}
	\begin{align}
	g^*(u\|q) = \log(1+q(e^u - 1)) \le q(e^u-1) \le q\left(u+\frac{u^2}{2}\right),
	\end{align}
	where the first inequality is from $\log(1+x)\le x$ for any $x>-1$, and the second inequality is from $e^x\le 
	1+x+x^2$ for any $x\le 0$.
\end{proof}

Using this property of the binary relative entropy, we decompose the expected instantaneous regret into two terms, which we will bound separately later.
In the following, let $\bar{\ell}_t(x,a) = \EV_{\theta \sim Q_t}[\ell(\theta,x,a)\vert \mathcal{F}_{t-1}]$ for any context $x$ and action 
$a$.

%Decoupling trick. This is general (does not assume noiseless binary losses)
\begin{lemma}
	For any $\eta>0$:\todo{We don't have further restrictions on $\eta$ because we only apply the duality trick to a 
negative term}
	\begin{equation}\label{eq:regret_decomp}
		\EV_t[r_t] \le \EV_t\left[\eta  g(\ell(\theta^\star,X_t,A_t) \| \bar{\ell}_t(X_t,A_t)) + 
\frac{1}{\eta}\sum_{a\in[K]}\bar{\ell}_t(X_t,a)\right].
	\end{equation}
\end{lemma}
\begin{proof}
	\todo{M: some passages can be omitted}
	\begin{align}
		\EV_t[r_t] 
		&=\EV\left[\ell(\theta^\star, X_t, A_t) - \ell(\theta^\star, X_t, A^\star_t)\mid\mathcal{F}_{t-1}\right] \nonumber\\
		&=\EV\left[\ell(\theta^\star, X_t, A_t) - \ell(\theta_t, X_t, 
A_t)\mid\mathcal{F}_{t-1}\right]\label{eq:ts_trick} \\
		&=\EV\left[\mathop{\EV}_{\theta^\star\sim Q_t}\left[\ell(\theta^\star, X_t, A_t)\mid\mathcal{F}_{t-1}, 
A_t\right] - \ell(\theta_t, X_t, A_t)\mid\mathcal{F}_{t-1}\right]\label{eq:tower} \\
		&=\EV\left[\mathop{\EV}_{\theta^\star\sim Q_t}\left[\ell(\theta^\star, X_t, A_t)\mid\mathcal{F}_{t-1}\right] - 
\ell(\theta_t, X_t, A_t)\mid\mathcal{F}_{t-1}\right]\label{eq:marginalize} \\
		&=\EV\left[\bar{\ell}_t(X_t, A_t) - \ell(\theta_t, X_t, A_t)\mid\mathcal{F}_{t-1}\right] \nonumber\\
		&= \EV_t\left[\bar{\ell}_t(X_t, A_t) - 
\sum_{a\in[K]}\mathbb{I}_{\{A_t=a\}}\frac{\eta\pi_t(a|X_t)}{\eta\pi_t(a|X_t)}\ell(\theta_t, X_t, a)\right]\nonumber\\
		&= \EV_t\left[\bar{\ell}_t(X_t, A_t) + \eta\sum_{a\in[K]}\pi_t(a|X_t)\left(g(\ell(\theta_t, X_t, 
a)\|\bar{\ell}(X_t,a)) 
\right.\right.\nonumber\\&\qquad+\left.\left. g^*\left(-\frac{\mathbb{I}_{\{A_t=a\}}}{\eta\pi_t(a|X_t)}\|\bar{\ell}(X_t, 
a)\right)\right)\right]\label{eq:fenchel_young} \\
		&\le \EV_t\left[\bar{\ell}_t(X_t, A_t) + \eta\sum_{a\in[K]}\pi_t(a|X_t)\left(g(\ell(\theta_t, X_t, 
a)\|\bar{\ell}(X_t,a)) - \frac{\mathbb{I}_{\{A_t=a\}}}{\eta\pi_t(a|X_t)}\bar{\ell}(X_t,a) 
\right.\right.\nonumber\\&\qquad+\left.\left.
\frac{\mathbb{I}_{\{A_t=a\}}}{2\eta^2\pi_t(a|X_t)^2}\bar{\ell}(X_t,a)\right)\right]\label{eq:dual_bound} \\
		&= \EV_t\left[ \eta\sum_{a\in[K]}\pi_t(a|X_t)g(\ell(\theta_t, X_t, a)\|\bar{\ell}(X_t,a)) + 
\sum_{a\in[K]}\frac{\mathbb{I}_{\{A_t=a\}}}{2\eta\pi_t(a|X_t)}\bar{\ell}(X_t,a)\right]\nonumber\\
		&= \EV_t\left[ \eta\sum_{a\in[K]}\pi_t(a|X_t)g(\ell(\theta_t, X_t, a)\|\bar{\ell}(X_t,a)) + 
\sum_{a\in[K]}\frac{\EV[\mathbb{I}_{\{A_t=a\}}\mid \mathcal{F}_{t-1}, X_t]}{2\eta\pi_t(a|X_t)}\bar{\ell}(X_t,a)\right]\nonumber\\
		&= \EV_t\left[ \eta\sum_{a\in[K]}\pi_t(a|X_t)g(\ell(\theta_t, X_t, a)\|\bar{\ell}(X_t,a)) + 
\frac{1}{2\eta}\sum_{a\in[K]}\bar{\ell}(X_t,a)\right]\nonumber\\
		&= \EV_t\left[ \eta\sum_{a\in[K]}\pi_t(a|X_t)g(\ell(\theta^\star, X_t, a)\|\bar{\ell}(X_t,a)) + 
\frac{1}{2\eta}\sum_{a\in[K]}\bar{\ell}(X_t,a)\right]\label{eq:ts_trick2}\\
		&= \EV_t\left[\eta g(\ell(\theta^\star, X_t, A_t)\|\bar{\ell}(X_t,A_t)) + 
\frac{1}{2\eta}\sum_{a\in[K]}\bar{\ell}(X_t,a)\right]\nonumber,
	\end{align}
	where~\eqref{eq:ts_trick} holds because, conditionally on $\mathcal{F}_{t-1}$, $(\theta^\star,A_t^\star)$ has the 
same distribution as $(\theta_t,A_t)$\todo{This TS trick should be commented in more detail somewhere.};
	\eqref{eq:tower} is by the tower rule of expectation;
	\eqref{eq:marginalize} is by conditional independence of $\theta^\star$ and $A_t$ given $\mathcal{F}_{t-1}$; 
\eqref{eq:fenchel_young} is from the Fenchel-Young inequality with convex function $g(\cdot\|\bar{\ell}(X_t,a))$; 
\eqref{eq:dual_bound} is from Proposition~\ref{prop:dual_bound} (note that $-\mathbb{I}_{\{A_t=a\}}/(\eta\pi_t(a|X_t))\le 0$ for any $\eta> 0$). Finally, \eqref{eq:ts_trick2} is again from $\theta^\star$ having the same distribution as $\theta_t$ conditional on $\F_{t-1}$.
\end{proof}

While the second term from the RHS of~\ref{eq:regret_decomp} can be easily bounded as $K/(2\eta)$, the relative entropy term requires more work. First, we rewrite it using a Bayesian-telescoping argument\todo{cit}.

\begin{lemma}\label{bayes_trick}
\begin{align*}
	&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} 
	= \EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\int_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})d\theta' }}.
\end{align*}
\end{lemma}

\begin{proof}
	Denoting the loss obtained in round $t$ by $L_t$ and noticing that $L_t \sim Ber(\ell(\theta^*, 
X_t, 
A_t))$, we get
	\begin{align*}
	&\EEt{g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} 
	\\
	&\qquad\qquad\qquad= \EEt{\ell(\theta^*, X_t, A_t) \log \frac{\ell(\theta^*, 
			X_t, A_t)}{\bloss_t(X_t, A_t)} + (1-\ell(\theta^*, X_t, A_t)) \log \frac{1-\ell(\theta^*, X_t, 
			A_t)}{1-\bloss_t(X_t, A_t)}}
	\\
	&\qquad\qquad\qquad=\EEt{p_{\theta^\star,t}(1)\log\frac{p_{\theta^\star,t}(1)}{\bar{p}_t(1)} + p_{\theta^\star,t}(0)\log\frac{p_{\theta^\star,t}(0)}{\bar{p}_t(0)}} \\
	&\qquad\qquad\qquad=\EEt{\EEs{\log\frac{p_{\theta^\star,t}(L_t)}{\bar{p}_t(L_t)} }{L_t\sim p_{\theta^\star,t}}}\\
	&\qquad\qquad\qquad=\EEt{\log\frac{p_{\theta^\star,t}(L_t)}{\bar{p}_t(L_t)}},
	\end{align*}
	where in the last step we introduced the notation $p_{\theta,t}(c) = \PPcc{ \mbox{Ber}\pa{\ell(\theta,X_t,A_t)}= 
		c}{X_t,A_t}$ and $\overline{p}_t(L_t) = \int_{\theta} q_t(\theta) p_{\theta,t}(L_t)d\theta$. Here, $q_t$ denotes the 
	posterior distribution over the parameter $\theta^*$.
	Then, summing up 
	and taking marginal expectations, we get
	\begin{align*}
		&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} 
		= \EE{\sum_{t=1}^T \EEt{ \log \frac{p_{\theta^*,t}(L_t)}{\overline{p}_t(L_t)}}}
		= \EE{\sum_{t=1}^T \log \frac{p_{\theta^*,t}(L_t)}{\overline{p}_t(L_t)}}
		\\
		&= \EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\prod_{t=1}^T \overline{p}_t(L_t)}}
	\end{align*}
	Let $d_{1:t}\in\{0,1\}^t$ be an element of the set of realizations of $L_{1:t}$ and $d_s$ is the $s$th coordinate of $d_{1:t}$. Let  $q_{L_{1:t}}(d_{1:t})$ denote a density of $L_{1:t}$ and let $q_t(\theta, d_{1:t})$ denote a joint density of $\theta^*$ and $L_{1:t}$. To proceed, let us notice that for any $d_t \in \{0,1\}^t$ the posterior updates take the following form by definition:
	\begin{align*}
		q_{t+1}(\theta) &= q_{\theta^*|L_{1:t} = d_{1:t} }(\theta) = \frac{q_{t}(\theta, d_{1:t}) 	}{q_{L_{1:t}}(d_{1:t})} 
		\\
		& = \frac{q_{t }(\theta, d_{1:t})}{\int_{\theta'}q_{t}(\theta', d_{1:t})d\theta'}
		\\
		& = \frac{q_{t}(\theta, d_{1:t-1}) p_{\theta,t}(d_t)}{\int_{\theta'}q_{t-1}(\theta', d_{1:t-1})p_{\theta',t}(d_t) d\theta' } 
		\\
		& = \frac{q_{t}(\theta) p_{\theta,t}(d_t)}{\int_{\theta'} q_{t}(\theta') p_{\theta',t}(d_t)d\theta'},
	\end{align*}
	where the last step follows from multiplying and dividing by the normalization constant of $q_t(\theta)$.
	Also, let us define the notation $\overline{p}(d_{1:T}) = \int_{\theta} q_0(\theta) \prod_{t=1}^T p_{\theta,t}(d_{t})$ 
	and notice that we can express this quantity by a recursive application of the above expression as 
	\begin{align*}
		\overline{p}(d_{1:T}) &= \prod_{t=1}^T \frac{\overline{p}(d_{1:t})}{\overline{p}(d_{1:t-1})}
		\\
		&= \prod_{t=1}^T \frac{\int_{\theta} q_0(\theta) \prod_{k=1}^t p_{\theta,k}(d_k) d\theta}{\int_{\theta'} q_{0}(\theta') 
			\prod_{k=1}^{t-1} p_{\theta',k}(d_k) d\theta'}
		\\
		&= \prod_{t=1}^T \int_\theta q_t(\theta) p_{\theta,t}(d_t) d\theta
		\\
		&= \prod_{t=1}^T \overline{p}_t(d_t).
	\end{align*}
	Then, we have
	\begin{align*}
		\EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\prod_{t=1}^T \bp_t(L_t)} } &= \EE{\log \frac{\prod_{t=1}^T 
				p_{\theta^*,t}(L_{t})}{\overline{p}(L_{1:T})} }
		= \EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\int_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})d\theta'}}.
	\end{align*}
\end{proof}

When $\Theta$ is a countable set, we can easily bound the relative-entropy term with the entropy of the prior distribution.

\begin{lemma} Let $Q_0$ be a distribution over countable set $\Theta$ with  bounded entropy, so for $\theta^* \sim Q_0$, $H(\theta^*) <\infty$. Then,
	\begin{align*}
	&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} \le H(\theta^*).
	\end{align*}
\end{lemma}
\begin{proof}
	Using the result of Lemma\ref{bayes_trick}, we can bound
	
	\begin{align*}
	&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} = \EE{ \log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\sum_{\theta'} Q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})}}\\
	&\qquad \le \EE{  \log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{Q_0(\theta^*) \prod_{t=1}^T p_{\theta^*,t}(L_{t})}  } = \EE{ - \log Q_0(\theta^*)} = H(\theta^*).
	\end{align*}
\end{proof}

%MOVED to Sec 3, delete when safe
%Since the entropy is not bounded for many discrete distributions that are of practical interest, and this result is not applicable to continuous distributions, we develop a more general result, that holds for broader family of distributions. In order to do so, we  need to make some assumptions on the distribution of the losses and on the support of $Q_0$. Let $\Theta$ be a support of $Q_0$.  For simplicity, we assume that $\Theta \subset \real^d$ and for any $\theta \in \Theta$, $\norm{\theta} \le 1$. We are making the following assumption on $p_{\theta,t}$:
%\begin{assumption}\label{log_lipshitz}
%	For any  $\theta, \theta' \in \Theta$, 
%	$\abs{\log p_{\theta,t}(L_t) - \log p_{\theta',t}(L_t)} \le C \norm{\theta - \theta'}$ holds for all 
%	$x,a$. 
%\end{assumption}
%This assumption may seem quite restrictive, but it holds for logistic regression. This  is referred as logistic bandits in the sequential learning literature \redd{[references]}. 
%\paragraph{Logistic bandits.}
%Let $L_t(\theta, x, a) \sim Ber(\sigma(f_{\theta}(x,a)) )$, where $\sigma(f_{\theta}(x,a)) = \frac{1}{1+ \exp(-f_{\theta}(x,a) )}$ and $f_{\theta}(x,a)$ is $L$-Lipschitz in $\theta$. Then $\log(\sigma(f_{\theta}(x,a))) = f_{\theta}(x,a) - \log(1+\exp(f_{\theta}(x,a)))$. Since $\log(\sigma(z))$ and $\log(1-\sigma(z))$ are $1$-Lipschitz, $\log(\sigma(f_{\theta}(x,a)))$ and $\log(1-\sigma(f_{\theta}(x,a)))$ are $L$-Lipschitz. 
%
%More general, Assumption~\ref{log_lipshitz} holds for any functions with a range within $(0,1)$: \paragraph{Bounded functions} More general, for any  $L$-Lipschitz function $f_{\theta}(x,a)$ with a range $[a,b]$ \todo{J: still that odd thing that $p_\theta(L_t)$ cannot be small} for some $0<a\le b<1$, $\log(f_{\theta}(x,a))$ and $\log(1 - f_{\theta}(x,a))$ are $\max \{\frac{1}{a}, \frac{1}{1-b}\} L$-Lipschitz.
%
%Before we prove our result for more general $Q_0$, we need to introduce some notations.   
%Let set $\hat{\Theta}_{\varepsilon}\subset \Theta$ be an $\varepsilon$-cover of set $\Theta$, so for any $\theta \in \Theta$ there exists $\hat{\theta} \in \hat{\Theta}_{\varepsilon}$, such that $\norm{\theta - 
%	\htheta} \le \varepsilon$. For any $\varepsilon$-cover, we can introduce a partition $\bar{\Theta}_{\varepsilon}$ of a set $\Theta$, and for any $\theta \in \Theta$ we denote $\bar{\Theta}_{\varepsilon}(\theta)$ a partition set containing $\theta$. Note that $|\bar{\Theta}_{\varepsilon}| \le |\hat{\Theta}_{\varepsilon}|$, as for any cover set we can assign a partition by associating every $\theta \in \Theta$ to the closest $\hat\theta \in \hat{\Theta}_{\varepsilon}$.  We let $\mathcal{N}_\varepsilon(\Theta,\norm{\cdot})$ denote the $\varepsilon$-covering number of $\Theta$. Then, 
%denoting the $\varepsilon$-ball around $\theta$ as $B_\varepsilon(\theta) = \ev{\htheta \in \Theta: \norm{\theta - 
%		\htheta} \le \varepsilon}$, we can easily see that the following holds for any $\theta$ and $\ttheta\in 
%B_\varepsilon(\theta)$: $\abs{\log p_{\theta,t}(L_t) - \log p_{\htheta,t}(L_t)} \le C \varepsilon$.

When $\Theta\subset\Reals^d$, we can still bound the relative-entropy term under Assumption~\ref{log_lipshitz} on the Lipschitz continuity of the log-likelihood.
First, we need to introduce some more notation.   
Let set $\hat{\Theta}_{\varepsilon}\subset \Theta$ be an $\varepsilon$-cover of set $\Theta$, so for any $\theta \in \Theta$ there exists $\hat{\theta} \in \hat{\Theta}_{\varepsilon}$, such that $\norm{\theta - 
	\htheta} \le \varepsilon$. For any $\varepsilon$-cover, we can introduce a partition $\bar{\Theta}_{\varepsilon}$ of a set $\Theta$, and for any $\theta \in \Theta$ we denote $\bar{\Theta}_{\varepsilon}(\theta)$ a partition set containing $\theta$. Note that $|\bar{\Theta}_{\varepsilon}| \le |\hat{\Theta}_{\varepsilon}|$, as for any cover set we can assign a partition by associating every $\theta \in \Theta$ to the closest $\hat\theta \in \hat{\Theta}_{\varepsilon}$.  We let $\mathcal{N}_\varepsilon(\Theta,\norm{\cdot})$ denote the $\varepsilon$-covering number of $\Theta$. Then, 
denoting the $\varepsilon$-ball around $\theta$ as $B_\varepsilon(\theta) = \ev{\htheta \in \Theta: \norm{\theta - 
		\htheta} \le \varepsilon}$, we can easily see that the following holds for any $\theta$ and $\ttheta\in 
B_\varepsilon(\theta)$: $\abs{\log p_{\theta,t}(L_t) - \log p_{\htheta,t}(L_t)} \le C \varepsilon$.

\begin{lemma}
	Under Assumption~\ref{log_lipshitz}, 
	$\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} \le d \log(2T+1) + C.$
\end{lemma}
\begin{proof}
	
	
	For any $\ttheta \in \Theta$: 
	\begin{align*}
		-\log \pa{\int_\theta q_0(\theta) \prod_{t=1}^T p_{\theta,t}(L_{t}) d\theta} &\le -\log 
		\pa{\int_{\bar{\Theta}_\varepsilon(\ttheta)} 
			q_0(\theta) \prod_{t=1}^T p_{\theta,t}(L_{t})d\theta}
		\\
		& = -\log \pa{\int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) \prod_{t=1}^T 
			\pa{p_{\ttheta,t}(L_{t})\cdot \frac{p_{\theta,t}(L_{t})}{p_{\ttheta,t}(L_{t})}}d\theta}
		\\
		&\le -\log \pa{\int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) \prod_{t=1}^T 
			\pa{p_{\ttheta,t}(L_{t})\cdot e^{-C\varepsilon}}d\theta}
		\\
		&\le -\log \pa{\int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) \prod_{t=1}^T 
			p_{\ttheta,t}(L_{t}) d\theta} + C\varepsilon T
		\\
		&= -\log \pa{S_0(\bar{\Theta}_\varepsilon(\tilde{\theta})) \prod_{t=1}^T  p_{\ttheta,t}(L_{t})} + C \varepsilon T,
	\end{align*}
	where we denoted $S_0(\bar{\Theta}_\varepsilon(\tilde{\theta})) = \int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) d\theta$. Using this calculation together with Lemma~\ref{bayes_trick}, we get
	\begin{align*}
		\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))}
		&=\EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\int_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})d\theta' }}
		\\
		&\le \EE{ \log \frac{p_{\theta^*} (L_{1:T})}{S_0(\bar{\Theta}_\varepsilon(\theta^*)) p_{\theta^*}(L_{1:T})}} + C \varepsilon T = \EE{ - \log 
			S_0(\bar{\Theta}_\varepsilon(\theta^*))} + C \varepsilon T
		\\
		&=-\int_{\theta}q_0(\theta) \log 
		S_0(\bar{\Theta}_\varepsilon(\theta))  + C \varepsilon T\\
		&= - \sum_{s \in \bar{\Theta}} S_0(s)  \log 
		S_0(s)  + C\varepsilon T 
		\\
		&\le \log\pa{\mathcal{N}_\varepsilon(\Theta,\norm{\cdot}) } + C\varepsilon T,
	\end{align*}
	where the last step is due to the fact that discrete uniform distribution maximizes the entropy among all discrete distributions with the same support.  
	Using a standard result on covering numbers (e.g. ..) that $\mathcal{N}_\varepsilon(\Theta,\norm{\cdot}) \le (\frac{2}{\varepsilon}+1)^d$  and taking $\varepsilon = 1/T$ gives the statement of the lemma. 
\end{proof}

==> 5-entropy.tex <==
\subsection{A general bound for the relative entropy loss (draft)}
Let us now attempt to bound the key terms in the bound: the sum of $\EEt{g(\ell(\theta^*, X_t, A_t) \| 
	\bloss_t(X_t,A_t))}$. 
\begin{lemma}\label{bayes_trick}
	\begin{align*}
		&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} 
		= \EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\int_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})d\theta' }}.
	\end{align*}
\end{lemma}

\begin{proof}
	Denoting the loss obtained in round $t$ by $L_t$ and noticing that $L_t \sim Ber(\ell(\theta^*, 
	X_t, 
	A_t))$, we get
	\begin{align*}
		&\EEt{g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} 
		\\
		&\qquad\qquad\qquad= \EEt{\ell(\theta^*, X_t, A_t) \log \frac{\ell(\theta^*, 
				X_t, A_t)}{\bloss_t(X_t, A_t)} + (1-\ell(\theta^*, X_t, A_t)) \log \frac{1-\ell(\theta^*, X_t, 
				A_t)}{1-\bloss_t(X_t, A_t)}}
		\\
		&\qquad\qquad\qquad= \EEt{\II{L_t=1} \log \frac{\ell(\theta^*, 
				X_t, A_t)}{\bloss_t(X_t, A_t)} + \II{L_t=0} \log \frac{1-\ell(\theta^*, X_t, 
				A_t)}{1-\bloss_t(X_t, A_t)}}
		\\
		&\qquad\qquad\qquad= \EEt{ \log \frac{p_{\theta^*,t}(L_t)}{\overline{p}_t(L_t)}},
	\end{align*}
	where in the last step we introduced the notation $p_{\theta,t}(c) = \PPcc{ \mbox{Ber}\pa{\ell(\theta,X_t,A_t)}= 
		c}{X_t,A_t}$ and $\overline{p}_t(L_t) = \int_{\theta} q_t(\theta) p_{\theta,t}(L_t)d\theta$. Here, $q_t$ denotes the 
	posterior distribution over the parameter $\theta^*$ for some realization of  $L_{1:t}$.
	Then, summing up 
	and taking marginal expectations, we get
	\begin{align*}
		&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} 
		= \EE{\sum_{t=1}^T \EEt{ \log \frac{p_{\theta^*,t}(L_t)}{\overline{p}_t(L_t)}}}
		= \EE{\sum_{t=1}^T \log \frac{p_{\theta^*,t}(L_t)}{\overline{p}_t(L_t)}}
		\\
		&= \EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\prod_{t=1}^T \overline{p}_t(L_t)}}
	\end{align*}
	
	Let $d_{1:t}\in\{0,1\}^t$ denotes a realization of $L_{1:t}$ and $d_s$ is the $s$th coordinate of $d_{1:t}$. Let  $q_{L_{1:t}}(d_{1:t})$ denote a density of $L_{1:t}$ and let $q_t(\theta, d_{1:t})$ denote a joint density of $\theta^*$ and $L_{1:t}$. To proceed, let us notice that for any $d_t \in \{0,1\}^t$ the posterior updates take the following form by definition:
	\begin{align*}
		q_{t+1}(\theta) &= q_{\theta^*|L_{1:t} = d_{1:t} }(\theta) = \frac{q_{t}(\theta, d_{1:t}) }{q_{L_{1:t}}(d_{1:t})} 
		\\
		& = \frac{q_{t }(\theta, d_{1:t})}{\int_{\theta'}q_{t}(\theta', d_{1:t})d\theta'}
		\\
		& = \frac{q_{t}(\theta, d_{1:t-1}) p_{\theta,t}(d_t)}{\int_{\theta'}q_{t-1}(\theta', d_{1:t-1})p_{\theta',t}(d_t) d\theta' } 
		\\
		& = \frac{q_{t}(\theta) p_{\theta,t}(d_t)}{\int_{\theta'} q_{t}(\theta') p_{\theta',t}(d_t)d\theta'},
	\end{align*}
	where the last step follows from multiplying and dividing by the normalization constant of $q_t(\theta)$.
	Also, let us define the notation $\overline{p}(d_{1:T}) = \int_{\theta} q_0(\theta) \prod_{t=1}^T p_{\theta,t}(d_{t})$ 
	and notice that we can express this quantity by a recursive application of the above expression as 
	\begin{align*}
		\overline{p}(d_{1:T}) &= \prod_{t=1}^T \frac{\overline{p}(d_{1:t})}{\overline{p}(d_{1:t-1})}
		\\
		&= \prod_{t=1}^T \frac{\int_{\theta} q_0(\theta) \prod_{k=1}^t p_{\theta,k}(d_k) d\theta}{\int_{\theta'} q_{0}(\theta') 
			\prod_{k=1}^{t-1} p_{\theta',k}(d_k) d\theta'}
		\\
		&= \prod_{t=1}^T \int_\theta q_t(\theta) p_{\theta,t}(d_t) d\theta
		\\
		&= \prod_{t=1}^T \overline{p}_t(d_t).
	\end{align*}
	Then, we have
	\begin{align*}
		\EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\prod_{t=1}^T \bp_t(L_t)} } &= \EE{\log \frac{\prod_{t=1}^T 
			p_{\theta^*,t}(L_{t})}{\overline{p}(L_{1:T})} }
		= \EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\int_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})d\theta'}}.
	\end{align*}
\end{proof}
\begin{lemma} Let $Q_0$ be a distribution over countable set $\Theta$ with  bounded entropy, so for $\theta^* \sim Q_0$, $H(\theta^*) <\infty$. Then,
	\begin{align*}
		&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} \le H(\theta^*).
	\end{align*}
\end{lemma}
\begin{proof}
	Using the result of Lemma\ref{bayes_trick}, we can bound
	
	\begin{align*}
		&\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} = \EE{ \log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\sum_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})}}\\
		&\qquad \le \EE{  \log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{q_0(\theta^*) \prod_{t=1}^T p_{\theta^*,t}(L_{t})}  } = \EE{ - \log q_0(\theta^*)} = H(\theta^*).
	\end{align*}
\end{proof}

Since the entropy is not bounded for many discrete distributions that are of practical interest, and this result is not applicable to continuous distributions, we develop a more general result, that holds for broader family of distributions. In order to do so, we  need to make some assumptions on the distribution of the losses and on the support of $Q_0$. Let $\Theta$ be a support of $Q_0$.  For simplicity, we assume that $\Theta \subset \real^d$ and for any $\theta \in \Theta$, $\norm{\theta} \le 1$. We are making the following assumption on $p_{\theta,t}$:
\begin{assumption}\label{log_lipshitz}
	For any  $\theta, \theta' \in \Theta$, 
 $\abs{\log p_{\theta,t}(L_t) - \log p_{\theta',t}(L_t)} \le C \norm{\theta - \theta'}$ holds for all 
	$x,a$. 
\end{assumption}
This assumption may seem quite restrictive, but it holds for logistic regression. This  is referred as logistic bandits in the sequential learning literature \redd{[references]}. 
\paragraph{ Logistic bandits.}
Let $L_t(\theta, x, a) \sim Ber(\sigma(f_{\theta}(x,a)) )$, where $\sigma(f_{\theta}(x,a)) = \frac{1}{1+ \exp(-f_{\theta}(x,a) )}$ and $f_{\theta}(x,a)$ is $L$-Lipschitz in $\theta$. Then $\log(\sigma(f_{\theta}(x,a))) = f_{\theta}(x,a) - \log(1+\exp(f_{\theta}(x,a)))$. Since $\log(\sigma(z))$ and $\log(1-\sigma(z))$ are $1$-Lipschitz, $\log(\sigma(f_{\theta}(x,a)))$ and $\log(1-\sigma(f_{\theta}(x,a)))$ are $L$-Lipschitz. 

More general, Assumption~\ref{log_lipshitz} holds for any functions with a range within $(0,1)$. \paragraph{Bounded functions} More general, for any  $L$-Lipschitz function $f_{\theta}(x,a)$ with a range $[a,b]$ \todo{J: still that odd thing that $p_\theta(L_t)$ cannot be small} for some $0<a\le b<1$, $\log(f_{\theta}(x,a))$ and $\log(1 - f_{\theta}(x,a))$ are $\max \{\frac{1}{a}, \frac{1}{1-b}\} L$-Lipschitz.

Before we prove our result for more general $Q_0$, we need to introduce some notations.   
 Let set $\hat{\Theta}_{\varepsilon}\subset \Theta$ be an $\varepsilon$-cover of set $\Theta$, so for any $\theta \in \Theta$ there exists $\hat{\theta} \in \hat{\Theta}_{\varepsilon}$, such that $\norm{\theta - 
	\htheta} \le \varepsilon$. For any $\varepsilon$-cover, we can introduce a partition $\bar{\Theta}_{\varepsilon}$ of a set $\Theta$, and for any $\theta \in \Theta$ we denote $\bar{\Theta}_{\varepsilon}(\theta)$ a partition set containing $\theta$. Note that $|\bar{\Theta}_{\varepsilon}| \le |\hat{\Theta}_{\varepsilon}|$, as for any cover set we can assign a partition by associating every $\theta \in \Theta$ to the closest $\hat\theta \in \hat{\Theta}_{\varepsilon}$.  We let $\mathcal{N}_\varepsilon(\Theta,\norm{\cdot})$ denote the $\varepsilon$-covering number of $\Theta$. Then, 
denoting the $\varepsilon$-ball around $\theta$ as $B_\varepsilon(\theta) = \ev{\htheta \in \Theta: \norm{\theta - 
\htheta} \le \varepsilon}$, we can easily see that the following holds for any $\theta$ and $\ttheta\in 
B_\varepsilon(\theta)$: $\abs{\log p_{\theta,t}(L_t) - \log p_{\htheta,t}(L_t)} \le C \varepsilon$.

\begin{lemma}
	$\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))} \le d \log(2T+1) + C.$
\end{lemma}
\begin{proof}


For any $\ttheta \in \Theta$: 
\begin{align*}
  -\log \pa{\int_\theta q_0(\theta) \prod_{t=1}^T p_{\theta,t}(L_{t}) d\theta} &\le -\log 
\pa{\int_{\bar{\Theta}_\varepsilon(\ttheta)} 
q_0(\theta) \prod_{t=1}^T p_{\theta,t}(L_{t})d\theta}
\\
& = -\log \pa{\int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) \prod_{t=1}^T 
\pa{p_{\ttheta,t}(L_{t})\cdot \frac{p_{\theta,t}(L_{t})}{p_{\ttheta,t}(L_{t})}}d\theta}
\\
&\le -\log \pa{\int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) \prod_{t=1}^T 
\pa{p_{\ttheta,t}(L_{t})\cdot e^{-C\varepsilon}}d\theta}
\\
&\le -\log \pa{\int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) \prod_{t=1}^T 
p_{\ttheta,t}(L_{t}) d\theta} + C\varepsilon T
\\
&= -\log \pa{S_0(\bar{\Theta}_\varepsilon(\tilde{\theta})) \prod_{t=1}^T  p_{\ttheta,t}(L_{t})} + C \varepsilon T,
\end{align*}
where we denoted $S_0(\bar{\Theta}_\varepsilon(\tilde{\theta})) = \int_{\bar{\Theta}_\varepsilon(\tilde{\theta})} q_0(\theta) d\theta$. Using this calculation together with Lemma~\ref{bayes_trick}, we get
\begin{align*}
\EE{\sum_{t=1}^T g(\ell(\theta^*, X_t, A_t) \| \bloss_t(X_t,A_t))}
 &=\EE{\log \frac{\prod_{t=1}^T p_{\theta^*,t}(L_{t})}{\int_{\theta'} q_0(\theta') \prod_{t=1}^T p_{\theta',t}(L_{t})d\theta' }}
 \\
 &\le \EE{ \log \frac{p_{\theta^*} (L_{1:T})}{S_0(\bar{\Theta}_\varepsilon(\theta^*)) p_{\theta^*}(L_{1:T})}} + C \varepsilon T = \EE{ - \log 
S_0(\bar{\Theta}_\varepsilon(\theta^*))} + C \varepsilon T
\\
&=-\int_{\theta}q_0(\theta) \log 
S_0(\bar{\Theta}_\varepsilon(\theta))  + C \varepsilon T\\
&= - \sum_{s \in \bar{\Theta}} S_0(s)  \log 
S_0(s)  + C\varepsilon T 
\\
&\le \log\pa{\mathcal{N}_\varepsilon(\Theta,\norm{\cdot}) } + C\varepsilon T,
\end{align*}
where the last step is due to the fact that discrete uniform distribution maximizes the entropy among all discrete distributions with the same support.  
Using a standard result on covering numbers (e.g. ..) that $\mathcal{N}_\varepsilon(\Theta,\norm{\cdot}) \le (\frac{2}{\varepsilon}+1)^d$ \todo{J: how it scales with the diameter of $\Theta$? } and taking $\varepsilon = 1/T$ gives the statement of the lemma. 
\end{proof}


